Walking Randomly, Massively, and Efficiently

We introduce a set of techniques that allow for efficiently generating many independent random walks in the Massive Parallel Computation (MPC) model with space per machine strongly sublinear in the number of vertices. In this space-per-machine regime, many natural approaches to graph problems struggle to overcome the $\Theta(\log n)$ MPC round complexity barrier. Our techniques enable breaking this barrier for PageRank---one of the most important applications of random walks---even in more challenging directed graphs, and for approximate bipartiteness and expansion testing. In the undirected case, we start our random walks from the stationary distribution, which implies that we approximately know the empirical distribution of their next steps. This allows for preparing continuations of random walks in advance and applying a doubling approach. As a result we can generate multiple random walks of length $l$ in $\Theta(\log l)$ rounds on MPC. Moreover, we show that under the popular 1-vs.-2-Cycles conjecture, this round complexity is asymptotically tight. For directed graphs, our approach stems from our treatment of the PageRank Markov chain. We first compute the PageRank for the undirected version of the input graph and then slowly transition towards the directed case, considering convex combinations of the transition matrices in the process. For PageRank, we achieve the following round complexities for damping factor equal to $1 - \epsilon$: * in $O(\log \log n + \log 1 / \epsilon)$ rounds for undirected graphs (with $\tilde O(m / \epsilon^2)$ total space), * in $\tilde O(\log^2 \log n + \log^2 1/\epsilon)$ rounds for directed graphs (with $\tilde O((m+n^{1+o(1)}) / poly\, \epsilon)$ total space).

==> 400-app-connectivity.tex <==
\section{Connectivity and MST}
\label{sec:ConnectivityAndMST}
In this section we will show how sampling random walks can be applied to construct an additive
$\epsilon n$ approximation for the number of connected components in the graph. Our algorithm
will require $O(\log \epsilon^{-1})$ rounds. We are going to use the following theorem that
shows how many vertices a length $l$ random walk will visit.

\begin{theorem}[\cite{Barnes:1993}]
For any connected graph on $n$ vertices and for any $N\le n$ the expected time
that a random walk visits $N$ distinct vertices is $CN^3$ for some constant $C$.
\end{theorem}

\begin{algorithm}[H]
\begin{algorithmic}[1]
\State{Using \cref{alg:random-walks} sample walks of length $2C(\epsilon^{-1}+1)^{3}$ in $G$.}
\State{$c \gets 0$}
\ForAll{$v \in V$ in parallel}
    \State{Let $s$ be the maximum number of distinct vertices visited by any walk starting in $v$.}
    \If{$s\le \epsilon{-1}$}
			\State{$c\gets c+1/s$.}
		\EndIf
\EndFor
\State{Return $c$.}
\end{algorithmic}
\caption{An algorithm computing $\epsilon n$ additive approximation to the number of components in graph $G$.}
\label{alg:random-c}
\end{algorithm}

\begin{theorem}
With probability at least $1 - \frac{2}{n}$, \cref{alg:random-c} computes $\epsilon n$ additive approximation to the number of components in graph $G$.
\end{theorem}
\begin{proof}
Consider a component $C$ of size $\le \epsilon^{-1}$. By Markov inequality with probability at least $1/2$ a random walk of length $2C\epsilon^{-3}\le 2C(\epsilon^{-1}+1)^{3}$ will visit all vertices
in $C$. As we have at least $\lceil 16\ln{n}\rceil$ walks starting in each vertex $v\in C$, with probability at least $1-n^{-15}$ one of the walks starting in $v$ will
visit all the vertices in $C$. In such a case $v$ will contribute  $1/|C|$ to $c$.

Now consider a component $C$ of size $>\epsilon^{-1}$. By Markov inequality with probability at least $1/2$ a random walk of length $2C(\epsilon^{-1}+1)^{3}$ will visit more than $\epsilon^{-1}$ vertices. As we have at least $\lceil 16\ln{n}\rceil$ walks starting in each vertex $v\in C$, with probability at least $1-n^{-15}$ one of the walks starting in $v$ will
visit more than $\epsilon^{-1}$ vertices. In such a case $v$ will contribute nothing to $c$.

By union bound over all the vertices the above events will happen with probability at least $1-n^{-14}$. By taking union bound with the success of \cref{alg:random-walks}
we get the probability of success to be $1-\frac{2}{n}$.
In such case vertices of components not larger than $\epsilon^{-1}$ contribute $1$, whereas
vertices of larger component contribute $0$. As there are no more than $n\epsilon$ components of size $>\epsilon^{-1}$ the theorem follows.
\end{proof}

The running time of the algorithm and the space requirement follow from \cref{lemma:ref-space-1}. Computing the number of
visited vertices by a walk requires sorting them, and this can be done in constant number of rounds~\cite{goodrich2011sorting}.

\begin{corollary}
   \cref{alg:random-c} works in $O(\log \epsilon^{-1})$ rounds and requires  $O(\epsilon^{-3} \log \epsilon^{-1} m \log n)$ space.
\end{corollary}

In~\cite{Chazelle:2005:AMS:1072890.1077946} the following $\epsilon$-approximation algorithm for the weight of minimum spanning tree was given.
This algorithm can be parallelized in a straight forward way.  We assume that we are given a connected graph $G=(V,E)$ where edges have integer weights $w:E\to [1\ldots W]$.
And let $G_i=(V,E_i)$ be the subgraph of $G$ which includes only edges of weight $\le i$.

\begin{algorithm}[H]
\begin{algorithmic}[1]
\State{$C_0\gets |V|$.}
\ForAll{$i =1,\ldots, W-1$ in parallel}
    \State{Let $C_i$ be the result of running \cref{alg:random-c} on $G_i$ with approximation $\frac{\epsilon}{2W}$.}
\EndFor
\State{Return $-W+\sum_{i=0}^{W-1} C_i$.}
\end{algorithmic}
\caption{An algorithm for computing $\epsilon$ approximation to the weight of MST in a connected graph $G$.}
\label{alg:random-mst}
\end{algorithm}

Using the analysis from~\cite{Chazelle:2005:AMS:1072890.1077946} we obtain the following.

\begin{theorem}
With probability at least $1 - \frac{2W}{\epsilon n}$, \cref{alg:random-mst} computes $(1+\epsilon)$-approximation to MST weight in a connected graph $G$.
The algorithm works in $O(\log (W\epsilon^{-1}))$ rounds and requires total space $O(W^4 \epsilon^{-4} \log (W\epsilon^{-1}) m \log n)$.
\end{theorem}

We note that the above result included just to show usefulness of the procedure for generating random walks. Having it at hand it is easy to
get additive approximation to the number of connected component. However, using standard PRAM algorithms for connectivity we can obtain the same
$O(\log (W\epsilon^{-1}))$ time but with less space. Consider for example the random-mate algorithm by Reif~\cite{Reif:1985}. This algorithm with constant
probability in each parallel round merges constant fraction of vertices into their neighbors. By running this algorithm for $O(\log (W\epsilon^{-1}))$
rounds all components of size at most $W\epsilon^{-1}$ will be merged into single vertices. This way additive approximation
to connected components requires $O(m+W\epsilon^{-1} n)$ space, whereas approximating MST can be done in $O(m+(W\epsilon^{-1})^2 n)$ space.


